Chiplet Cloud: Building AI Supercomputers for Serving Large Generative Language Models

Large language models (LLMs) such as OpenAI's ChatGPT and Google's Gemini have demonstrated unprecedented capabilities of autoregressive AI models across multiple tasks triggering disruptive technology innovations around the world. However, as models continue to grow the cost to serve these models also continues to grow threatening the democratization of LLMs. To address this issue, we propose Chiplet Cloud, a chiplet-based ASIC LLM-supercomputer architecture whose goal is to optimize the total cost of ownership (TCO) per generated token. This architecture is a highly parameterizable ASIC and server-level architecture leveraging thousands of replicated accelerator modules collaborating to scale-up the performance of LLMs at cloud-scale. To determine specific parameterizations of the Chiplet Cloud architecture, we implemented a two-phase hardware-software co-design methodology that can search the massive design space and fine tune the architecture across a collection of LLMs based on an accurate inference simulation. A common bottleneck for LLMs is the memory access performance therefore we introduce CC-MEM, a scalable on-chip memory system for Chiplet Cloud architectures. Using the CC-MEM, Chiplet Clouds can be built using only SRAMs for design points where the power and performance of memory access is critical. The CC-MEM also includes a compression decoder module to add support for sparse models without impacting the compute units using a Store-as-Compressed, Load-as-Dense mechanism. We evaluate Chiplet Cloud architectures across eight popular LLMs. Using fine tuned Chiplet Cloud servers we are able to achieve $97\times$ and $18\times$ improvement in TCO/Token over rented GPU and TPU clouds, or a $8.3\times$ and $3.7\times$ improvement over fabricated GPU and TPU clouds respectively. Chiplet Cloud can also support $1.7\times$ larger models with a sparsity of 60\%.

==> HPCA_TEXT.tex <==
\newpage
\part{HPCA Submission}
\setcounter{section}{0}

\section{Introduction}
\label{sec:intro}

In recent years, transformer-based language models \cite{vaswani_attention_2017, devlin_bert_2019, liu_roberta_2019, raffel_exploring_2020} have fueled the rapid progress in Natural Language Processing (NLP).
Leveraging the transformer block, language models such as BERT~\cite{devlin_bert_2019} provide significant performance improvements over conventional recurrent neural networks. 
As large-scale computation and large datasets becoming more available, large language model \cite{radford_language_2019, noauthor_turing-nlg_2020, brown_language_2020, fedus_switch_2021} are becoming more popular.
These language models achieve unprecedented accuracy at unprecedented scale.
The number of parameters in state-of-the-art language models have grown exponentially as shown in Fig.~\ref{fig:model_size}.
As a result of the exponential growth rate, these models cost huge amount of hardware resource.
For example, GPT-3~\cite{brown_language_2020} with 175B parameters requires 23 days to train on 1536 A100 GPUs \cite{narayanan_efficient_2021}.
It's also getting more expensive to run these models.
The original transformer~\cite{vaswani_attention_2017} can be deployed on a single GPU, while the GPT-3 requires an NVIDIA DGX A100 server that includes 8 A100 GPUs.
With the end of Moore's Law, transistor size scaling slows down and the fabrication yield issue grows.
Building large monolithic chips to address these massive workloads has become increasingly expensive.
Hardware cost will limit the impact of large models.
We need a more scalable and economical hardware architecture for large language models.

\begin{figure}
    \centering
    \includegraphics[width=0.42\textwidth]{img/model_size.pdf}
    \caption{
    The number of parameters in language models grows exponentially at a rate of about $10\times$ per year.
    }
    \label{fig:model_size}
\end{figure}



Transformer-based language models also run extremely slow on GPUs.
For example, GPT-2~\cite{radford_language_2019} with 1.5B parameters takes a second to generate 20 tokens on a V100 GPU.
One reason for the long latency is that these language models contain a large number of fully connected (FC) operations, which have low operational intensity and require high parameter bandwidth.
Figure~\ref{fig:roofline} shows the roofline of GPT-2 on a V100 GPU, where most kernels are bounded by the memory bandwidth.
To fully utilize the 112 TFLOPS computing power on V100, we need a total bandwidth of 85000 GB/s, which is about $100\times$ of HBM bandwidth.
Meanwhile, low operational intensity and large model size also make the DRAM access dominates the energy consumption.
Reducing parameter access latency and power is critical for large language models.

To address the above challenges, we propose Chiplet Cloud, a cloud-scale chiplet architecture for large language models, which aims to (1) deliver state-of-the-art performance, while (2) reducing the fabrication cost and total-cost-of-ownership (TCO) compared to current GPU-based systems.
We use \emph{performance/cost} and \emph{performance/TCO} as key metrics to define the design space of Chiplet Clouds.

Chiplet technology has recently become a new trend in the industry.
It breaks down a traditional monolithic silicon chip into multiple small chiplets and integrates them into a single package.
This approach improves fabrication yield, reduces manufacturing costs and enables die-level reuse for different system scales.
However, the performance of chiplet systems is often limited by inter-chiplet communication.
We observe that a transformer layer can be divided into stages with the same amount of parameters and operations, and there is little traffic between those stages.
This motivates us to combine the chiplet approach with \textit{pipeline parallelism} \cite{huang_gpipe_2019,kosson_pipelined_2021,yang_pipemare_2020,gao_tangram_2019} at the layer or stage level to reduce communication between chiplets.
We further extend the definition of chiplet from package-level to board-level to alleviate the design challenges posed by package-level integration.
Chiplet Clouds use the same chiplet on the same package, but with different board designs, are able to support different language models efficiently.
Board-level chiplet architecture also offers better scalability than GPUs and package-level chiplets. 

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{img/roofline.pdf}
    \caption{
    Roofline of GPT-2 on a V100 GPU. Most kernels have low operational intensity and are bandwidth (HBM) bounded.
    To reach the ridge point with the same computing power, it requires about $100\times$ bandwidth.
    }
    \label{fig:roofline}
\end{figure}


To address bandwidth bottleneck issue and improve performance, we propose to buffer all model parameters on-chip.
On-chip memories such as SRAM have better read latency and read energy than external memories such as DDR or HBM, but require more silicon.
We show this design choice wins in the competition of performance per TCO for large language models.

In summary, this paper makes the following contributions:
\begin{enumerate}
    \item We conduct comprehensive characterizations on the transformer-based language models, which motivates us the use of chiplet and large on-chip memory.
    \item We propose Chiplet Cloud, a chiplet-based cloud-scale architecture for large language models to improve performance and cost.
    \item We analyze and compare the trade-offs of different mapping strategies for large language models.
    \item We present a deign flow which explores the hardware design and model mapping space of Chiplet Cloud.
    \item We design and evaluate Chiplet Clouds on 4 popular models. 
    Compared to GPUs, evaluation results show a improvement in performance per TCO up to $490\times$.
\end{enumerate}




\section{Background and Motivation}
\label{sec:background}

\subsection{Transformer Architecture}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{img/layer.pdf}
    \caption{
    The transformer layer can be divided into 3 stages with roughly the same number of parameters and operations. 
    Only a few activations are transferred between stages.
    Sub-leading terms such as nonlinearities and biases are omitted.
    }
    \label{fig:layer}
\end{figure}

The transformer neural network architecture~\cite{vaswani_attention_2017} has became the backbone of many recent deep learning models~\cite{devlin_bert_2019, radford_language_2019, noauthor_turing-nlg_2020, brown_language_2020, liu_swin_2021} due to its superior performance.
The architecture of a transformer layer is shown in Figure~\ref{fig:layer}, which is replicated multiple times in the model.
The transformer layer is mainly composed of a multi-head self-attention mechanism and a 2-layer feed-forward network.
A detailed description of the transformer layer can be found in the original paper~\cite{vaswani_attention_2017}.

We characterize all main operations in a transformer layer, annotating the number of operations and parameters of each sub-modules in the middle of Figure \ref{fig:layer}.
Transformer layers are parameterized by the dimension of the residual stream $d_{model}$, the dimension of the feed-forward layer $d_{ff}$, and the dimension of the attention output $d_{attn}$.
Normally, we have $d_{model}=d_{attn}=d_{ff}/4$.
We denote this value as $d$ for simplicity.
When the model is used for a generative task, it first takes the input sequence as a whole and generates a word as output.
Then it uses that word as the next input, runs the model again and generates the next word.
It continues to do so until generating an end of text token.
Therefore, the input sequence length $l$ is always 1 during a text generation, except for the first run.
For large language models, the model dimension $d$ is usually larger than 10,000, so we have $O(ld^2)>>O(l^2d)$.
Fully connected (FC) layers have more operations than other modules such as scale or softmax in self-attention, and dominate the computation of the entire transformer layer.
For example, 99.56\% of MACs in GPT-3 are spent on FC.
In addition, most of the model parameters also come from the FC layer, causing a lot of memory accesses.
In this work, we mainly focus on the acceleration of FC layers.

We further observe the whole transformer layer can be partitioned in to 3 stages, \textit{Attention}, \textit{FC 0} and \textit{FC 1}, in terms of the needed operations and parameters. 
As shown on the right side in Figure~\ref{fig:layer}, each stage requires roughly the same number of parameters ($4d^2$) and the the same number of operations ($8ld^2$).  
Only a few activations ($2ld$ bytes or $8ld$ bytes) are transferred between stages.
We call these stages \emph{transformer stages}.
This observation motivates us to combine the use of chiplets with pipeline parallelism for large language models.
The model can be broken down into thousands of transformer layers or transformer stages, all requiring the same amount of computation and memory, and each map to a chiplet.
Thousands of chiplets then run the entire model in a pipelined fashion.
Intuitively, this setup not only provides good scalability, but also reduces inter-chip communication, which has been one of the biggest problems with chiplet systems.
Detailed analysis and evaluation will be described in the following sections.


\subsection{Design for Performance per TCO: All Parameters On-Chip}

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{img/mem_compare.pdf}
    \caption{Compared with DDR and HBM, SRAM has order-of-magnitude better bandwidth and read energy, leading to better \textit{perf/TCO} designs.
    }
    \label{fig:mem}
\end{figure}

Instead of just optimizing raw hardware performance, more companies start to design accelerators for better performance per TCO \cite{jouppi_ten_2021}.
TCO of an accelerator consists of the capital expense (\textit{CapEx}, mainly from chip fabrication) and the operation expense (\textit{OpEx}, mainly from power consumption), and the $TCO=CapEx+life\times OpEx$.
Consider a language model accelerator with die area of $area$ and average power of $power$, that provides a total parameter bandwidth of $BW$.
The accelerator's TCO can be approximately modeled as $\alpha \cdot area + \beta \cdot power$, where $\alpha$ and $\beta$ are constant coefficients.
\revise{Chip cost actually grows superlinearly with area. We use a linear model here for simplicity, which will not affect our subsequent analysis.} 
As indicated by Figure \ref{fig:roofline}, current single-node hardware is bandwidth bounded, performance will be proportional to the parameter bandwidth $BW$.
As a result, we have
$$\frac{perf}{TCO} \propto \frac{1}{\alpha \frac{area}{BW} + \beta \frac{power}{BW}}$$
To optimize the performance per TCO, we want a smaller $area/BW$ and $power/BW$.
Assuming that other modules in the chip remain unchanged, the area, read energy, and bandwidth of the the parameter memory will be key factors affecting this figure of merit.
We list typical memory blocks of DDR4, HBM2e and SRAM in the table in Figure~\ref{fig:mem}, and plot the area per total bandwidth and the read energy per total bandwidth when we use these blocks to store model parameters.
Compared with DDR and HBM, on-chip SRAM has much smaller $area/BW$ ($\frac{mm^2}{GB/s}$) and $power/BW$($\frac{pJ/bit}{GB/s}$).
Although the same memory technology can have blocks of different sizes, which affects bandwidth and read energy, the trend shown in Fig.~\ref{fig:mem}  remains the same, i.e. SRAM has an order-of-magnitude better area per bandwidth and read energy per bandwidth than DRAM.
This is because DRAM stores data in capacitors and needs periodic refreshment to maintain the charge, while SRAM stores data in transistors.
Thus, although buffering all parameters on-chip requires more silicon, it will likely lead to better performance per TCO designs.

Recently, there has been an industry trend to deploy more on-chip memory on deep learning accelerators to reduce external memory accesses.
Microsoft's Brainwave~\cite{fowers_configurable_2018} pins DNN model weights in distributed on-chip SRAM.
Google's TPUv4i \cite{jouppi_ten_2021} contains 144 MB SRAM, and GraphCore's IPU 2 \cite{knowles_graphcore_2021} has 896 MB SRAM,
\revise{Cerebaras WSE-2 \cite{systems_wafer-scale_2019} has a huge 18 GB on-chip memory}.
Adding more on-chip memory to provide higher bandwidth is easier, cheaper, and lower power than doubling the HBM bandwidth, which benefits the performance per TCO design orientation.


\section{Chiplet Cloud for Language Models}
\label{sec:cloud}

Over the past years, chiplet has become one of the promising methods to extend Moore's Law.
Instead of integrating more functionality per silicon chip, this approach designs and fabricates small chiplets and integrates those chiplets into one package \cite{kannan_enabling_2015, arunkumar_mcm-gpu_2017, naffziger_pioneering_2021}.
Compared to large monolithic chips, chiplets have much better fabrication yields, reducing manufacturing and testing costs.
It also enables a die-level reuse for different sizes of system.
It is especially suitable for emerging applications with various scales of repeat operations, such as language models.
Recently, NVIDIA proposes Simba \cite{shao_simba_2019, venkatesan_011_2019}, the first DNN accelerator using chiplet technology.
In this section, we introduce a chiplet-based cloud-scale system for language model, called \textit{Chiplet Cloud}.
We illustrate the Chiplet Cloud architecture, identify the design parameters and discuss the design challenges.

\subsection{Architecture of Chiplet Cloud}

A general Chiplet Cloud architecture is shown in Figure~\ref{fig:all_arch}, which includes the high-level abstract architecture of different levels, from process unit (PU) to chiplet, board, and cloud.
Starting from the bottom left, we start with the heart of Chiplet Cloud, a language model accelerator that scales to data center inference.
The chiplet adopts a frequently-used PU-based architecture, with additional attention, nonlinear function, and normalization units.
The Chiplet Cloud PU has a simple design, which only includes a parameter memory, multiple parallel MACs (multiply-accumulate) units, and an accumulation buffer.
Each MAC consists of a 16 bit Google's brain floating point (BFloat16) \cite{wang_bfloat16_2019} multiplication and a 32 bit single-precision floating-point (fp32) addition.
Model parameters are distributed in those PU parameter memories.
The input buffer reads activation from another chiplet or the host through a chip-to-chip (C2C) router and broadcasts it to all PUs. 
Thus, all PUs share the same activation inputs, but different weights from the local parameter memory.
Partial sums are accumulated inside each PU.
The dataflow and architecture are specifically designed for the FC operations in transformer, which includes more input reuse and less parameter reuse.
This is because the size of the parameter is much larger than the input, as we discussed in Section~\ref{sec:background}.
The design maximizes parallelization and eliminates the need for inter-PU communication, reducing on-chip network overhead.
The output of a PU either goes to the attention unit and then goes back to the PU array, or goes to some nonlinear units like GeLu and normalization and is sent outside the chip.

A key feature of a Chiplet Cloud is that a single chiplet is a package, multiple chiplets are connected through the board.
Conventionally, chiplets are integrated into a single package via a package-level solution such as a silicon interposer (such as \cite{kannan_enabling_2015}) or organic substrate (such as Simba~\cite{shao_simba_2019} and AMD EPYC processor\cite{naffziger_pioneering_2021}) for better inter-chiplet communication.
For instance, Simba achieves a 100 GB/s/chiplet bandwidth through the ground-referenced-signaling (GRS) technology \cite{zimmer_032128_2020, zimmer_011_2019}.
However, the package-level integration brings design challenges and overhead.
Silicon interposers have a limited signal length.
The organic substrate solution brings design challenges in package-level routing and power delivery~\cite{naffziger_pioneering_2021}.
Instead, we extend the definition of chiplet to \textit{board-level} in Chiplet Cloud according to the communication requirements.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{img/arch.pdf}
    \caption{
    High-Level Chiplet Cloud architecture.
    }
    \label{fig:all_arch}
\end{figure}


Since we decided to buffer all model parameters on-chip, activations are the only data that needs to be read off-chip.
With an optimized workload partitioning and mapping strategy, we can further reduce traffic across chiplets.
Chiplets have individual packages and are connected together via a customized on-PCB network. 
To accommodate the potential different mapping strategies for different language models, we just need to redesign the board and still reuse the same chiplet package.
The board-level chiplet architecture eliminates the need for high speed interfaces and reduces the nonrecurring engineering (NRE) cost of the package design.
In fact, according to our application study in Section~\ref{sec:studies}, 4 server designs with the same chiplet can efficiently support language models from GPT-2 \cite{radford_language_2019} with 1.5 billion parameters to Megatron-Turing NLG\cite{smith_using_2022} with 530 billion parameters.
Experiment results in Section~\ref{sec:design_exp} show the board-level chiplet architecture also benefits cooling, as heat generation is more evenly distributed across the board.

Each Chiplet Cloud server contains a printed circuit board (PCB) with multiple chiplets, a controller and an off-PCB interface. 
The controller, which can be an FPGA or a microcontroller, dispatches remote procedure calls (RPCs) from off-PCB interface to all chiplets via a customized on-PCB network.
The on-PCB network is a point-to-point interconnection for all chiplets.
Candidate interfaces are high speed PCI-e, which has been widely used as interconnects for many deep learning chips \cite{smelyanskiy_zion_2019, prabhakar_sambanova_2021, liu_ai_2021}, or custom-designed links such as Google TPU's Inter-Core Interconnect links \cite{jouppi_domain-specific_2020} and Graphcore's IPU-links \cite{knowles_graphcore_2021}.
Off-PCB interfaces could be 100 Gigbit Ethernet or InfiniBand, enabling communication between adjacent servers.

\subsection{Design Space}

Design space of a Chiplet Cloud includes chiplet design and system design.
Starting with the chiplet, we mainly need to determine the peak performance (in TOPS, depending on the number of MACs and clock frequency) and the size of the SRAM (in MB) of the chiplet.
Chiplet of different TOPS and SRAM sizes have different area and power consumption, affecting TCO and final performance.
Smaller chiplet designs improve the fabrication yield while adding more total silicon and more inter-chiplet communication.
We aim to design a chiplet with suitable size for language models of different scales.
Chiplet Cloud server design depends on the application.
Depending on how we partition and map the model, we customize the server, including the number of chiplets per server and the on-PCB network, as well as the total number of servers required.
We present an end-to-end design and evaluation flow in Section~\ref{sec:design_exp}.

\subsection{Challenges}

Recalling the goals we presented in Section~\ref{sec:intro}, we wanted to design a new system for large language models with better performance per cost or TCO.
The main insight of the Chiplet Cloud is the use of board-level chiplets to reduce hardware cost and all-parameter-on-chip to improve performance.
While these design choices benefit one of our goals, they also pose challenges for the other.
In the rest of this paper, we will answer the following two problems and justify the design of Chiplet Cloud.

\textit{Problem 1: Will performance be limited by inter-chip communication?}
Inter-chip communication has become one of the limitations of many GPU-based distributed deep learning systems \cite{li_pipe-sgd_2018, shoeybi_megatron-lm_2020}.
As we break down large DL chips into smaller chiplets, we add more chip-to-chip and even server-to-server communication.
We will show that a carefully chosen mapping strategy can significantly reduce off-chip traffic and that our customized inter-chiplet routing will meet the bandwidth requirements.

\textit{Problem 2: Will all-parameter-on-chip greatly increase cost?}
Storing all model parameters in on-chip memory instead of DRAM requires more silicon.
We argue that although this design choice increases hardware costs, the overall performance per cost and per TCO will still be better due to its large benefit to performance and power.


\section{Model Mapping In Chiplet Cloud}
\label{sec:map}

It is now standard practice to parallelize DNN across distributed heterogeneous clusters.
To maintain high device utilization and reduce inter-device communication in distributed systems with thousands of nodes, a proper mapping strategy is critical.
On GPU-based systems, various parallelism techniques such as \textit{data parallelism}, \textit{tensor model parallelism} and \textit{pipeline model parallelism} have been proposed~\cite{shazeer_mesh-tensorflow_2018,jia_beyond_2018,ben-nun_demystifying_2018,fedus_switch_2021}.
In this section, we compare different mapping strategies in Chiplet Cloud for language model inference.


\subsection{Parallelism Modes}

Data parallelism (DP) \cite{krizhevsky_imagenet_2012, li_pytorch_2020} places a copy of the entire model on each node so that each node processes a subset of the input batch.
Data parallelism is easy to implement, but it requires much more memory and is not be feasible for large models on Chiplet Cloud.
It is commonly used in large batched DNN training to improve the training throughput, while the batch size of inference tasks can be very small, in which case data parallelism cannot take advantage of all nodes.

Model parallelism \cite{dean_large_2012} is another common parallelism mode, which assigns disjoint subsets of a model each to a dedicated node.
Model parallelism saves memory for parameters, but typically requires more data transfers between nodes.
Depending on the partition dimension, there are tensor model parallelism and pipeline model parallelism.
In tensor model parallelism (TP, or tensor parallelism), individual layers of the model are partitioned over multiple nodes. 
Layers can be partitioned from either dimension of the layer parameters.
Since operations within a layer are also partitioned across nodes, TP requires frequently inter-node synchronization, such as partial sum accumulation and layer normalization.
In pipeline model parallelism (PP, or pipeline parallelism), disjoint subsets of layers are assigned to multiple nodes.
In a language model, each node is assigned the same number of transformer layers, and all nodes operate in a pipelined fashion.
Compared to tensor parallelism, pipeline parallelism eliminates most of the inter-node communication.

\begin{figure}
    \centering
    \includegraphics[width=0.50\textwidth]{img/PP.pdf}
    \caption{Example of using only pipeline model parallelism on Chiplet Cloud. Each chiplet is mapped to a transformer stage. 
    This minimizes the traffic between chiplets and servers.
    }
    \label{fig:PP}
\end{figure}

Pipeline parallelism is one of the main motivations for Chiplet Cloud.
It requires less memory than data parallelism and less inter-node traffics than tensor parallelism.
The idea is straightforward and easy to implement.
Based on our analysis from Figure~\ref{fig:layer}, we can extend PP to a more fine-grained stage-level to accommodate less memory per device.
Figure~\ref{fig:PP} shows an example of PP on Chiplet Cloud.
$W_*$ denote the weight of FC layers.
Each chiplet is assigned to just one transformer stage, and works as a pipeline stage in the whole system.
Three chiplets (or three transformer/pipeline stages) make up a transformer layer.
A server usually includes multiple layers, depending on the server size. 
This implementation minimizes inter-node traffic and requires only point-to-point communication.
However, pipeline parallelism tends to have longer latency than tensor parallelism because all nodes operate in a pipelined fashion.
The more pipeline stages, the longer the latency.
Furthermore, for very large models like GPT-3, 
there are over 600 million parameters for each transformer stage.
More than 1.2 GB of memory is required per transformer stage, which is not feasible for a single chiplet.
To accommodate large models, tensor parallelism is also essential in Chiplet Cloud.
The next problem becomes how to properly partition parameter tensors across chiplets.

\subsection{Tensor Partitioning Strategy in Detail}


\begin{figure}[t]
\subfloat[$A$ and $B$ are split by row, requiring two reduce \& scatter.]{%
  \includegraphics[clip,width=1.0\columnwidth]{img/map1.pdf}%
  \label{fig:map1}
}

 \centering
\subfloat[$A$ and $B$ are split by column, requiring two all-gather.]{%
  \includegraphics[clip,width=1.0\columnwidth]{img/map2.pdf}%
  \label{fig:map2}
}

 \centering
\subfloat[$A$ is split by row, $B$ is split by column, requiring one all-reduce.]{%
  \includegraphics[clip,width=1.0\columnwidth]{img/map3.pdf}%
  \label{fig:map3}
}

 \centering
\subfloat[$A$ is split by column, $B$ is split by row, requiring one all-reduce.]{%
  \includegraphics[clip,width=1.0\columnwidth]{img/map4.pdf}%
  \label{fig:map4}
}
\caption{Tensor partitioning strategies for consecutive GEMMs.
 $A\in \mathbb{R}^{C\times M}$ and $B\in \mathbb{R}^{M\times C}$ are two weight matrices.
All required collective operations are shown in the red box. 
% Links are annotated with the traffic. 
}
\label{fig:gemm_map}
\end{figure}

\begin{figure*}[]
 \centering
\subfloat[In this example, a server includes the entire layer. We modify the partitioning strategy from \cite{narayanan_efficient_2021}. The all-reduce operation in the last stage of the server is replaced by a reduce and a broadcast in the next server to reduce off-server traffic.]{%
  \includegraphics[width=0.88\textwidth]{img/PP_TP_1.pdf}%
  \label{fig:PP_TP_1}
}

 \centering
\subfloat[In this example, a server includes only one transformer stage, and 3 servers are concatenated to form a layer. The weight matrices in both FC1 and FC2 are split by column, eliminating synchronization between chiplets in Servers 2 and 3.]{%
  \includegraphics[width=0.95\textwidth]{img/PP_TP_2.pdf}%
  \label{fig:PP_TP_2}
}
\caption{
    In Chiplet Cloud, tensor model parallelism with different tensor partitioning strategies are combined with pipeline model parallelism.
    Depending on model size and chiplet size, Chiplet Clouds can employ different mapping strategies and inter-chip routing patterns.
    }
\end{figure*}

As shown in Figure~\ref{fig:layer}, a transformer layer consists of four FC layers, 2 in the multi-head self-attention (the 3 FC layers of $Q$, $K$ and $V$ are parallel and can be merged into one) and 2 in the feedforward network.
The parameters of these FC layers are two-dimensional matrices.
To analyze the partitioning strategy in tensor model parallelism, let's consider the following example with two consecutive matrix multiplications (GEMMs),$I=XA, Y=IB$.
$X,Y\in \mathbb{R}^{1\times C}$ are input and output, $A\in \mathbb{R}^{C\times M}$ and $B\in \mathbb{R}^{M\times C}$ are two weight matrices, and $I\in \mathbb{R}^{1\times M}$ is the intermediate result.
Weight matrix $A$ and $B$ can be partitioned either along their rows or columns.
Figure~\ref{fig:gemm_map} shows four different partitioning strategies can be applied.
Links between nodes are annotated with data traffic.

When both weight matrices are split in half by row (Figure~\ref{fig:map1}), each node takes half of the input and produces a partial sum. 
These partial sums need to be accumulated to get the result.
Therefore, partial sums are reduced ($(I_{psum}, I_{psum})\to I$) then scattered ($I \to (I_1, I_2)$) to different nodes between GEMM.
When both are split in half by column (Figure~\ref{fig:map2}), each node takes the entire input tensor and produces part of the result.
After each GEMM, an all-gather operation ($(I_1, I_2)\to (I, I)$) is required to collect and broadcast data across nodes .
Compared to the previous one, this method requires more input bandwidth while eliminating the synchronization of partial sum accumulation between nodes. 

Figure~\ref{fig:map3} shows a hybrid approach.
Matrix $A$ is split by row and matrix $B$ is split by column.
GEMM $XA$ takes half the input and produces partial sum, while $IB$ takes the entire input and produce half the output.
As a result, only one all-reduce operation ($(I_{psum}, I_{psum})\to (I, I)$) is required per two GEMMs.
The other data transfer can be directly connected.
These strategies seem to be advantageous compared to (a) and (b), since they only require one all-reduce per two GEMMs.
Megatron-LM \cite{shoeybi_megatron-lm_2020} first applies this tensor partitioning strategy to GPU clusters.
Later work \cite{narayanan_efficient_2021} combines it with pipeline parallelism and achieves state-of-the-art speeds for GPT-3 training.

These works choose tensor partitioning strategies based on experimental results on GPU clusters, which are not necessarily optimal for Chiplet Cloud.
For example, GPU implementations typically use smaller-sized pipeline parallelism, matrix multiplication $X_1A_1$ and $I_1B_1$ in Figure~\ref{fig:gemm_map} are in the same GPU node in most cases. 
Whereas in Chiplet Clouds, they are usually in different pipeline stages and different chiplet nodes, off-chip communication of intermediate results $I$ is unavoidable.
In this case, the all-gather operation in Figure~\ref{fig:map2} can be implemented through simple point-to-point links, which is cheaper than the all-reduce operation in Figure~\ref{fig:map3}.

\subsection{Chiplet Cloud Mapping Examples}

Chiplet Cloud can address more fine-grained parallelism modes and partitioning strategies than GPU cluster since it has more nodes of smaller size.
Additionally, customized chiplet-to-chiplet routing provides Chiplet Cloud with greater flexibility when mapping different models.
Combining model mapping and server design, Chiplet Cloud brings a new type of software-hardware co-design methodology.

Figure~\ref{fig:PP_TP_1} shows an example of when the server can map the entire transformer layer.
All required data collective operations across chiplets are shown in the red box.
We use the tensor partitioning strategy from \cite{shoeybi_megatron-lm_2020} and \cite{narayanan_efficient_2021} with some modification.
This approach adopts the strategy shown in Figure~\ref{fig:map3} in both self-attention and feedforward networks.
A major benefit of this approach is that it requires only two all-reduce operations per layer for inter-device communication.
Our implementation combines it with a stage-level pipeline parallelism to accommodate the chiplet design.
Each pipeline stage contains only one transformer stage, which is one third of the transformer layer.
We also customize the data transfer between servers.
We change all-reduce operation in the last stage in a server to a reduce operation and a broadcast operation in the next server.
This modification saves the bandwidth between servers because the tensor ($O$ in Figure~\ref{fig:PP_TP_1}) is only transferred once.
Duplicated operations in the last stage is also removed, such as \textit{Add\&Norm} in chiplet 5 in Figure~\ref{fig:PP_TP_1}.

As the model size continues to increase, the server may not be able to map the entire transformer layer.
Figure~\ref{fig:PP_TP_2} shows an example of a server containing only one transformer stage, and 3 servers are concatenated to form a layer.
Another different routing pattern and partitioning strategy is shown here.
The all-reduce operation in server 1 between chiplet 1 and 2 is changed to reduce operation to save off-server traffic.
The strategy in Figure~\ref{fig:map2} is used to partition the feedforward network (FC 1 and FC 2).
The all-gather operation in this strategy is implemented through the gather operation at the output end of the server and the broadcast operation at the input end.
Therefore, synchronization across chiplets is not required in servers 2 and 3.
This example reduces both inter-server and inter-chiplet communication.

\subsection{Chiplet Cloud Mapping Heuristics}
\label{sec:map_principle}

Based on the above analysis, we summarize some heuristics for mapping language models to Chiplet Cloud as follows:
\begin{enumerate}[itemsep=-0.1ex]
    \item \emph{Avoid tensor model parallelism across servers.} Collective operations brought by tensor parallelism require high bandwidth and should be avoided at the server level. Ideally, only pipeline parallelism should be used across servers.
    \item \emph{Generally, the tensor partitioning strategy in Figure~\ref{fig:PP_TP_1} is preferred.} It only requires two all-reduce operations per layer, reducing traffic between chiplets.
    \item \emph{The tensor partitioning strategy in Figure~\ref{fig:PP_TP_2} is preferred when the server contains only one GEMM.} Since the chiplet output in a server needs to be collected anyway before being sent out, this strategy eliminates synchronization between chiplets compared to Figure~\ref{fig:PP_TP_1}.
    \item \emph{Avoid all-reduce at the end of the server, use reduce instead.} Tensors are sent out of the server and do not need to up update in all chiplets.
\end{enumerate}

Note that these principles do not necessarily lead to the optimal strategy.
The performance of parallelism modes and partitioning strategy in Chiplet Cloud depends on various factors such as model size, chiplet computing power, and inter-chiplet bandwidth, all of which need to be considered when making choices. 
Chiplet cloud gives designers the flexibility to customize the interconnects of chiplets and servers, usually through point-to-point links without any switches.
Compared to GPUs server, interconnection in a Chiplet Cloud is specialized for the target model and partitioning strategy.
It eliminates unnecessary links between nodes and provides more bandwidth for the required links.
Studies and evaluation of real applications are discussed in Section~\ref{sec:studies}.

\section{Design of a Chiplet Cloud}
\label{sec:design_exp}

The design space of the chip cloud is much larger than that of the GPU clusters.
In this section, we introduce the design and evaluation flow of Chiplet Cloud.

\subsection{Overall Design and Evaluation Flow}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.42\textwidth]{img/flow.pdf}
    \caption{
    The Chiplet Cloud design evaluation flow consists of two parts.
    The chiplet design flow (red) generates an optimized accelerator chiplet design.
    The system design flow (blue) then finds the optimal mapping strategy and chiplet interconnect with the best performance or TCO for a specific model.
    }
    \label{fig:flow}
\end{figure}

The design space of the Chiplet Cloud consists of the chiplet itself and the cloud.
Chiplet Cloud tends to use just one accelerator chiplet design for multiple transformer-based language models.
Cloud level designs  are dedicated to target models and their mapping strategies.
Therefore, we divide the entire Chiplet Cloud design and evaluation process into two parts, chiplet design flow and system design flow, as shown in Figure~\ref{fig:flow}.
Optimization goals could be performance (throughput or latency), hardware cost, power, and TCO.

In chiplet design flow, the optimization goal is to find the chiplet design that achieves the highest \textbf{TOPS per cost, energy, or TCO of a server}.
This is by tuning the MAC array and the memory size in PU array.
Performance of language models also depends on the interconnects and model mapping, which are addressed in the system design flow. 
Given a chiplet design, the system design flow finds the Chiplet Cloud system design that optimizes the \textbf{model performance per cost or TCO for a particular model}.


\subsection{Chiplet Design}

While the chiplet approach has many potential advantages, it also introduces new costs.
Some functions need to be implemented on each chiplet, such as IOs, clock generation, power management, test and debug interfaces, and more.
In Chiplet Cloud, those also includes the inter-chiplet communication interfaces, attention and post-processing module.
As a result, a design with more smaller chiplets leads to better yield but requires more total silicon and more power consumption.
How to choose the right chiplet size is one of the main design challenges of chiplet systems, which is addressed in our chiplet design flow.

Inputs of the chiplet design flow include ASIC specs and server constraints.
Table~\ref{tab:inputs} shows detailed descriptions of the main inputs.
The flow generates and evaluates various chiplet designs with different computing performance and on-chip memory.
According to the optimization objective, it outputs the optimized chiplet design, which will be used for language models of different scales.
At this point, chiplet interconnects are ignored since the mapping strategies are unknown.
\revise{They will be addressed in the system design flow.}
Only the number of chiplets per server is considered in subsequent cooling and server evaluations.

\begin{table}[]
\centering
\caption{Inputs of the chiplet design flow.}
\label{tab:inputs}
\begin{tabular}{|l|l|}
\hline
\textbf{Inputs} & \textbf{Descriptions} \\ \hline
ASIC Specs &
  \begin{tabular}[c]{@{}l@{}}
  PU performance density (TOPS/mm$^2$) \\ 
  PU power density (W/mm$^2$)\\ 
  PU memory density (MB/mm$^2$)\\ 
  Other modules (\revise{controller, router, etc}) area (mm$^2$) \\
  Other modules power (W)
  \end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Server \\ Constraints\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}
  Chiplet lanes (\#) \\
  Chiplet area per lane  (\textless{}mm$^2$) \\
  Air Cooling Configurations (heat sink, fan, etc.) \\
  \end{tabular} \\ \hline
\end{tabular}
\end{table}

This cooling and server evaluation engine is built on the ASIC Cloud model~\cite{magaki_asic_2016, khazraee_moonwalk_2017} with the advanced nodes (7nm) added.
Similar to ASIC Cloud, we focus on the standard 1U 19-inch rackmount servers, all chiplets are placed in a DUCT layout on PCB.
The server uses a forced air cooling system to dissipate heat, 
\revise{with a fan employed in front of each lane.
The chiplet lanes constraint comes from server width and fan size per lane.}
The engine first calculates the chiplet specifications, including power, area, power, etc.
Based on the chiplet power and area per lane, it estimates the thermal profile and removes overheating designs.
The engine then calculates the total performance, power, and TCO of the server.

The TCO model is a refined version of the model by Barroso et al~\cite{barroso_datacenter_2013}, which includes datacenter capital expenditures (\emph{CapEx}) and operating expenses (\emph{OpEx}), server \emph{CapEx} and \emph{OpEx} and electricity cost.
\revise{To obtain server \emph{CapEx}, our server cost model considers die cost, package cost, PCB cost, power cost, cooling cost, etc.
The power cost includes cost of DC/DC converters and power supply units (PSU).}
The cooling cost includes cost of heatsinks and fans.
To estimate the die cost, we first calculate the number of fully patterned dies per wafer (DPW). 
Cost per die is than calculated by
$$cost_{die}=(\frac{cost_{wafer}}{DPW}+cost_{test})/Y_{die}$$
where ${cost_{wafer}}$ is wafer price 
, $cost_{test}$ is testing cost, and $Y_{die}$ is die yield.
We use the classical negative binomial model for yield as follow
$$Y_{die}=(1+\frac{AD_0}{\alpha})^{-\alpha}$$
where $A$ is die area, $D_0$ is defect density 
and $\alpha$ is cluster parameter.
Figure~\ref{fig:cost_model} shows the results of our die cost model for TSMC 7nm.
Since manufacturing yields drop with chip area, it makes economic sense to design smaller chips.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.40\textwidth]{img/cost_model.pdf}
    \caption{
    The fully patterned dies per wafer (DPW), die yield and die cost versus die area in TSMC 7nm.
    Chip cost grows super-linearly with area, which is the main driver of chiplet.
    }
    \label{fig:cost_model}
\end{figure}


\begin{figure}[b]
    \centering
    \includegraphics[clip,width=1.0\columnwidth]{img/chiplet_cost.pdf}
    \caption{How the number of chiplets per server affects the silicon cost of a server with the same total performance and memory. The appropriate chiplets size is essential for balancing yield and total area.
}
\label{fig:chiplet_size}
\end{figure}

We further show how the chiplet size affects the total silicon area and cost in a server in Figure~\ref{fig:chiplet_size}.
Given the fixed performance and memory requirements of a server, when we use smaller chiplets, more chiplets are required per server.
Smaller chips increase manufacturing yields and reduce silicon costs.
However, when chiplets become too small, per-chiplet circuits begin to dominate the the total area, resulting in even larger silicon costs.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.43\textwidth]{img/chiplet_exp.pdf}
    \caption{
    Chiplet design space exploration of servers with fixed total SRAM.
    Each point series show total TOPS per server and the number of chiplets increases from left to right points.
    The lower left points have better performance per TCO.
    }
    \label{fig:chiplet_exp}
\end{figure}

Using the chiplet design infrastructure we developed, we ran simulations exploring the design space of chiplet for a Chiplet Cloud server.
In Chiplet Clouds, we don't just optimize raw hardware performance or power, we care about two metrics: cost efficiency, defined by hardware cost per performance (\$ per TOPS), and energy efficiency, defined by energy per operation (joules per tera-ops, equivalent to watts per TOPS).
Designers can optimize just one of these metrics, or they can find the TCO-optimal point by properly balancing the importance of cost efficiency and energy efficiency.
Figure~\ref{fig:chiplet_exp} shows the energy efficiency versus cost efficiency Pareto of Chiplet Cloud servers.
All designs utilize 7 nm technology.
\revise{Inputs of Table~\ref{tab:inputs} come from real 7nm DL accelerator designs, such as TPU v4i~\cite{jouppi_ten_2021} and GraphCore IPU 2~\cite{knowles_graphcore_2021}.
For instance, the PU performance density is set as 3.45 TOPS/mm$^2$.}
Our simulations evaluate servers with varying numbers of chiplets and total compute performance (TOPS) and prune those that violate system requirements.
Each point series shows total server TOPS and the number of chiplets increases from 16 on the far left to 160 on the far right.
Adding more MACs to increase total TOPS will always result in both better \$ per TOPS and watts per TOPS as long as thermal requirements are met, because a higher ratio of silicon and power are used for computation.
As we shrink the chiplet size and have more chiplets per server, \$ per TOPS initially decreases with better manufacturing yields and lower hardware costs, but eventually chiplet overhead area starts to dominate, the total cost begins to rise.
Meanwhile, this also increases watts per TOPS, as per-chiplet circuits add more power.


Table~\ref{tab:chiplet_opt} shows the points for energy and cost efficiency optimized designs.
The energy-optimal server has a larger die size, 538 mm$^2$, which minimizes the chiplet power consumption overhead.
The cost-optimal server 
adopts a smaller chiplet design, 148 mm$^2$, to increase fabrication yield and reduce the total silicon cost.
Table~\ref{tab:chiplet_opt} also shows TCO optimal server based on our TCO model, which has die size and performance in between cost- and energy-optimal designs.
All designs support chiplet-to-chiplet bandwidths up to 50 GB/s.
We employ the TCO optimal chiplet design in the following system design flow.

\begin{table}[b]
\centering
\caption{Chiplet design optimization results.}
\label{tab:chiplet_opt}
\begin{tabular}{|l|r|r|r|}
\hline
 & \textbf{Energy Opt.} & \textbf{Cost Opt.} & \textbf{TCO Opt.} \\
\hline
TOPS / chiplet       &   87.5 &   21.9 &   43.8 \\ \hline
MB / chiplet         &    720 &    180 &    360 \\ \hline
Die Size (mm$^2$)    &    538 &    148 &    280 \\ \hline \hline
\# chiplets / server &     16 &     64 &     32 \\ \hline
\revise{W / TOPS}      & \revise{\textbf{1.52}}     & \revise{1.59}   & \revise{1.54} \\ \hline
\revise{\$ / TOPS}            & \revise{2.77}     & \revise{\textbf{2.34}}   & \revise{2.41} \\ \hline
\revise{TCO / TOPS}           & \revise{9.12}     & \revise{8.94}   & \revise{\textbf{8.81}} \\ \hline

\end{tabular}
\end{table}


\subsection{System Design}

After the chiplet design is finalized, a system design flow is performed for each model to generate the complete Chiplet Cloud system, including model mapping and server design.

Fine-grained mapping is the key module in the system design flow.
Given a model and a chiplet design, it generates all possible mappings, including the parallelism modes and tensor partitioning strategies.
Specifically, the parallelism mode can be represented as two values $p$ and $t$.
$p$ is the pipeline model parallel size and $t$ is the tensor model parallel size.
We require $p \cdot t$ to be equal to the total number of chiplets.
Tensor partitioning is only applied when $t>1$.
The parameter tensor of each GEMM can be split either along its columns or rows. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.42\textwidth]{img/map_example.pdf}
    \caption{
    Model mapping and server design.
    In this example, the 6-chiplet-server is mapped to 1 transformer layer (3 transformer stages), and the server parallelism mode is $t=2, p=3$.
    The tensor partition strategy is shown at the top.
    Arrows are point-to-point chiplet interconnects.
    The data flow order and size are marked on the arrows.
    }
    \label{fig:map_example}
\end{figure}

The corresponding server design for each mapping is then generated.
Suppose a transformer layer is assigned to the server with 6 chiplets in the initial partitioning.
Figure~\ref{fig:map_example} shows a fine-grained mapping example that uses the same strategy as Figure~\ref{fig:PP_TP_1}.
It includes not only model mapping, but also all required chiplet interconnects.
In a Chiplet Cloud server, all interconnections are through point-to-point links, including collective operations.
In this example, link \circled{2} and \circled{3} execute \emph{broadcast}, link \circled{4} and \circled{5} execute \emph{all-reduce}, and link \circled{8} executes \emph{reduce}.
When the tensor parallel size becomes larger, more chiplets are involved in the collective operations, requiring more complicated interconnections.
Among all parallel algorithms for broadcast, reduce and gather, 
we prefer the linear pipeline approach since each node is only required to connect to the neighbor nodes, reducing both the number of wires and total wire length on PCB.
We adopts the \emph{ring all-reduce} algorithm for all-reduce collective, which has been widely used in neural network training on GPU clusters.
All involved nodes are connected into a ring to perform the ring all-reduce.

In system design flow, an analytical model is used to evaluate the performance of Chiplet Cloud for a specific application.
Based on the mapping and interconnection information, the model first analyzes the data traffic of each link, as shown in Figure~\ref{fig:map_example}, and calculates the data transmission time according to the link bandwidth.
Since all model parameters are buffered on the chiplet, parameter bandwidth will no longer be the bottleneck.
The execution time of chiplets can be estimated by the computation time, which are obtained from the mapped operations and the TOPS of the chiplet.
Based on data transfer time, chiplet execution time, and data dependencies, the model calculates server latency and throughput.
Overall chiplet system latency is the sum of all server latency plus data transfer time between servers.
All of this performance information, along with the server TCO, will be used to help us choose the system that meets our needs.

\begin{table}[b]
\centering
\caption{Target models and systems.}
\label{tab:target_model}

\begin{tabular}{|l|r|r|r||r|r|}
\hline
\textbf{Model} & \textbf{$d$} & \textbf{Layers}  & \textbf{Total Size} & \textbf{Chips/Srv.} & \textbf{\# Srv.} \\ \hline \hline
GPT-2      &  1600 &  48 &   2.9 GB &  9 &   1 \\ \hline
Turing NLG &  4256 &  78 &    34 GB & 28 &   4 \\ \hline
GPT-3      & 12288 &  96 &   348 GB & 36 &  32 \\ \hline
MT-NLG     & 20480 & 105 &  1057 GB & 30 & 105 \\ \hline
\end{tabular}

\end{table}

\subsection{Case Studies}
\label{sec:studies}

We design and evaluate Chiplet Cloud on four language models, which are GPT-2\cite{radford_language_2019} and GPT-3\cite{brown_language_2020} proposed by OpenAI,
and Turing NLG\cite{noauthor_turing-nlg_2020} and Megatron-Turing NLG (MT-NLG) \cite{smith_using_2022} proposed by Microsoft and NVIDIA.
To accommodate the different model sizes, we adjust the number of chiplets per server and calculate the number of servers required.
Dimensions of these models and systems are shown in Table \ref{tab:target_model}.


\subsubsection{Mapping}

To find the optimal fine-grained mapping for models, we ran simulations exhaustively evaluating all possible parallelism modes and tensor partitioning strategies.
Among all tensor partitioning strategies, the same one as Figure~\ref{fig:PP_TP_1} outperforms all others, conforming to the second point of Section~\ref{sec:map_principle}.
Figure~\ref{fig:p_modes} shows how different parallelism modes affect the end-to-end latency.
The parallelism mode can be represented as pipeline-parallel size $p$ and tensor-parallel size $t$, $p \cdot t$ is equal to the total number of chiplets used.
As $p$ increases, there will be more pipeline stages.
At the same time, as $t$ decreases, fewer chiplets run in parallel for each pipeline stage, resulting in less inter-chiplet communication.

\begin{figure}[t]
    \centering
    \includegraphics[trim=0 0 0 0, clip, width=0.45\textwidth]{img/p_modes.pdf}
    \caption{
    End-to-end latency of various parallelism modes for 4 target models.
    The optimal modes are marked in red.
    Large pipeline-parallel sizes increase pipeline stages while reducing the amount of data transfer between nodes.
    Balancing the tradeoff between pipeline and tensor parallel size is important to achieve better latency.
    }
    \label{fig:p_modes}
\end{figure}

In GPT-2 systems, the one maximizes tensor parallelism and minimizes pipeline parallelism has the smallest latency.
This is because it requires only 1 server with 9 chiplets, inter-chiplet communication does not introduce much delay.
All 48 layers are housed in these 9 chiplets and run in one pipeline stage.
The Turing NLG system requires 4 servers, each containing 28 chiplets.
The evaluation results show that a parallelism mode of $(p=8, t=14)$ minimizes the latency.
The model is split into 8 pipeline stages, each stage has 14 chiplets and fits 10 transformer layers (the last one fits 8).
As shown in Figure \ref{fig:p_modes}, the latency-optimal parallelism modes of GPT-3 and MT-NLG are $(p=32, t=36)$ and $(p=105, t=30)$. 
The pipeline parallel sizes are equal to the desired server number, respectively.
Tensor model parallelism for all these models only happens on chiplets in the same server, conforming to the first point of Section~\ref{sec:map_principle}.

\subsubsection{Model-Specific Server}
\revise{Fig.14 motivates us to design model-specific servers that ensures high performance and utilization across different models.}
The server designs for Turing NLG and Megatron-Turing NLG are shown in Figure \ref{fig:server_designs}.
Each Turing NLG server has 28 chiplets and are divided into 2 pipeline stages to fit 20 layers.
To perform the required collective operations, such as \emph{all-reduce}, the chiplets in each pipeline stage are connected in a ring.
Turing NLG requires 4 servers in total.
For MT-NLG, all 30 chiplets in a server are run in one pipeline stage to fit 1 layer.
They are connected in a ring to perform collective operations.
MT-NLG requires a total of 105 such servers for 105 layers.
Servers for GPT-2 and GPT-3 have the same interconnect as the MT-NLG server, with 9 and 36 chiplets each, respectively.

\begin{figure}[b]
    \centering
    \includegraphics[width=.47\textwidth]{img/servers.pdf}
    \caption{Server designs for Turing-NLG and Megatron-Turing NLG using the same chiplet.}
    \label{fig:server_designs}
\end{figure}

\begin{table*}[]
\centering
\caption{Compare Chiplet Cloud to GPU servers.}
\label{tab:compare}
\begin{tabular}{|l|l|r|r|r|r|r|r|r|r|}
\hline
Models &
  Systems &
  \begin{tabular}[c]{@{}r@{}}Cost\\  (\$)\end{tabular} &
  \begin{tabular}[c]{@{}r@{}}Power\\   (W)\end{tabular} &
  \begin{tabular}[c]{@{}r@{}}TCO \\ (\$)\end{tabular} &
  \begin{tabular}[c]{@{}r@{}}Latency \\ (ms)\end{tabular} &
  \begin{tabular}[c]{@{}r@{}}Throughput\\ (tokens/s)\end{tabular} &
  % \begin{tabular}[c]{@{}r@{}}Throughput\\ per TCO\end{tabular} &
  \begin{tabular}[c]{@{}r@{}}$Perf$/TCO\end{tabular} &
  \begin{tabular}[c]{@{}r@{}}$Perf$/TCO \\ Improvement\end{tabular} \\
  % Increase &
  \hline \hline
 &
  1 Chiplet Cloud server &
  1.2 K &
  0.5 K &
  3.4 K &
  0.02 &
  49,356 &
  639,630 &
   \\ \cline{2-8} 
\multirow{-2}{*}{GPT-2} &
  1 A100 GPU &
  19 K &
  0.4 K &
  22 K &
  1.5  &
  105,263 &
  3,140 &
  \multirow{-2}{*}{229$\times$} \\ \hline
 &
  4 Chiplet Cloud servers &
  12 K &
  6.6 K &
  40 K &
  0.092 &
  43 K &
  10,778 & \\ \cline{2-8} 
\multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}Turing \\ NLG\end{tabular}} &
  1 A100 GPU &
  19 K &
  0.4 K &
  22 K &
  17 &
  9.2 K &
  24 &
  \multirow{-2}{*}{490$\times$}  \\ \hline
 &
  32 Chiplet Cloud servers &
  120 K &
  68 K &
  403 K &
  0.5 &
  65 K &
  169 &
  \\ \cline{2-8} 
\multirow{-2}{*}{GPT-3} &
  1 DGX server (8 A100 GPUs) &
  149 K &
  3.2 K &
  179 K &
  21.9 &
  7.2 K &
  1.8 &
  \multirow{-2}{*}{174$\times$}  \\ \hline
 &
  105 Chiplet Cloud servers &
  354 K &
  198 K &
  1.2 M &
  1.6 &
  66 K &
  32.1 &
  \\ \cline{2-8} 
  \multirow{-2}{*}{MT-NLG} &
  2 DGX servers (16 A100 GPUs) &
  298 K &
  6.4 K &
  358 K &
  33.1 &
  4.7 K &
  0.02 &
  \multirow{-2}{*}{85$\times$}  \\ \hline
\end{tabular}
\end{table*}


\section{Evaluation}
\label{sec:evaluation}

In this section, we evaluate the cost, performance and TCO of Chiplet Clouds through design choice sanity checks and comparisons with GPU systems.

Latency and throughput are two important performance metrics for language models.
Latency affects user experience, and throughput determines how many tokens can be processed per unit time.
To compare these two metrics at the same time, we define the metric $Perf=throughput/latency$.
The larger the $Perf$, the better the overall performance.

The analytical model in our design flow is used to evaluate latency and throughput.
The model takes into account not only computing power, but also different bandwidths between chips and servers, as well as pipeline bubbles, collective operation latency~\cite{chan_collective_2007}, etc.
All designs are in TSMC 7nm. 
Fabrication costs are estimated from real wafer price \cite{sole_price_2020} and density  \cite{cutress_better_2020}.


\subsection{Design Choice Sanity Checks}

To demonstrate the benefits of our design choices, including all model parameters on the chip and board-level chiplets without advanced interconnect technology, we compare Chiplet Cloud with two systems.
The first system employs a traditional HBM-based architecture (HBM) with all parameters stored in DRAM.
\revise{The silicon interposer (SI) is only used in HBM in this system.
The second system pins model parameters on the chip while using SI to enable inter-chip communication .}
Multiple chiplets are integrated into one package through SI, and a server contains multiple packages.
We use the model from \cite{stow_cost_2016} to estimate the cost of SI. 
Design space exploration for both systems is performed using our flow.
Figure \ref{fig:si_hbm_pareto} shows the power and cost efficiency pareto for Chiplet Cloud and two systems.
Compared to SI and HBM, our system has better power per TOPS and cost per TOPS.
This is mainly because both HBM and SI bring additional manufacturing cost and power consumption without contributing to computing performance.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.35\textwidth]{img/si_hbm.pdf}
    \caption{
    Compared to systems with silicon interposer and HBM, Chiplet Cloud has better cost and power efficiency because of its simpler architecture.
    }
    \label{fig:si_hbm_pareto}
\end{figure}

\begin{figure}[b]
    \centering
    \includegraphics[width=0.46\textwidth]{img/si_hbm_app.pdf}
    \caption{
    Latency, throughput and performance per cost comparison for all target models.
    Chiplet Cloud outperforms HBM and silicon interposer systems.
    All data are normalized to HBM.
    }
    \label{fig:si_hbm_app}
\end{figure}

We further compare the performance of 4 language models that we presented in Figure~\ref{fig:si_hbm_app}.
The optimal HBM and SI systems are used.
Compare to HBM system, Chiplet Cloud improves the latency by $95\times$, throughput by $23\times$ and $Perf$/cost by $220$ on average.
We also observe SI systems have slightly worse performance than Chiplet Cloud.
Due to the large size of these models, requiring hundreds to thousands of chiplets and packages, inter-package communication is unavoidable.
High in-package bandwidth does not help much for large model inference.
Additionally, because the chiplets with silicon interposers are closer to each other, heat generation is more concentrated on the board, reducing maximum allowable power and performance.
Chiplet Cloud achieves a $1.4\times$ better $Perf$/cost than SI systems on average.

\subsection{Comparisons with GPUs}

In Table~\ref{tab:compare}, we compare Chiplet Clouds versus GPU-based servers.
For a fairness comparison, we only consider the power of chiplets and GPU in our TCO model.
We show that this architecture greatly improves performance and $Perf/$TCO.
Chiplet Clouds outperform GPUs on $Perf/$TCO by $229\times$, $490\times$, $174\times$, and $85\times$ for GPT-2, Turing NLG, GPT-3 and Megatron-Turing NLG, respectively. 


\subsection{Cost of Chiplet Cloud}

Compared to current GPU systems, the added TCO of Chiplet Cloud is the result of orders-of-magnitude better performance. 
Current business model of large language models is to charge by the number of input tokens. 
Because of the limited performance of GPU systems, only a limited number of tokens can be run per day. 
Chiplet Cloud significantly improves inference performance, helping companies gain priority in the growing NLP market.
It also enables powerful large language models to be used in more fields.

Another major factor limiting the deployment of ASIC accelerators on the cloud is non-recurring engineering (NRE) costs.
The NRE of Chiplet Clouds includes mask cost, labor, CAD tools, IP licensing, flip-chip BGA packing, server designs, etc.
According to the model of Moonwalk~\cite{khazraee_moonwalk_2017}, we estimate the NRE of 7nm Chiplet Clouds to be \revise{\$33.5M}, most of which comes from the mask cost.
The global NLP market size is expected to reach \$127.26B by 2028 according to Fortune Business Insights~\cite{noauthor_natural_2021}. One key feature of large LMs is that once trained, they can be deployed on various tasks with little fine-tuning and run continuously for long periods of time.
Chiplet Cloud is proposed based on the insight that most large LMs (GPT-3 \cite{brown_language_2020}, MT-NLG \cite{smith_using_2022} and the latest PaLM \cite{chowdhery_palm_2022}) are all based on the similar architecture, but with different sizes and training methods. 
Our chiplet supports all operations in the transformer and can run all models efficiently in a scale-up manner. 
Board-level chiplets offer better scalability than GPUs.
The NRE of each application-specific server are around \revise{\$8M, which consists of DL stack design (\$6M), PCB, FPGA and other hardware design (\$2M).
They are estimated based on the latest engineer salary~\cite{noauthor_glassdoor_2022}.
Server hardware design for different applications doesn't add much NRE.
We assume a server life of 1.5 years, which is a conservative assumption compare to LM lifetime. 
Released more than two years ago, GPT-3 is still one of the most well-known and popular LMs.
We believe there will be sufficient market and lifetime to justify the NRE.
}

\subsection{\revise{Chiplet Clouds vs. ASIC Clouds}}
\revise{
Chiplet Clouds and ASIC Clouds~\cite{magaki_asic_2016} are different. 
ASIC Clouds are for scale-out workloads such as cryptocurrency mining and video transcoding, that consist of many independent but similar jobs.
Chiplet Clouds are for scale-up workloads, large language models, where computations are tightly-coupled.
Compared to ASIC Clouds, this work provides a detailed analysis of different model mapping strategies and customized on-PCB networks.
}


\section{Related Work}
\label{sec:rela}

\cite{kannan_enabling_2015} and \cite{arunkumar_mcm-gpu_2017} are two of the pioneer work leveraging chiplet technology in CPU and GPU.
Recently, Simba \cite{shao_simba_2019, venkatesan_011_2019} implements the first 36-chiplet prototype multi-chip-modules (MCM) system for deep learning inference.
NN-Baton \cite{tan_nn-baton_2021} proposes a framework to explore the chiplet design space for convolutional NN.
All of this work is focused on chiplets in a single package.

Accelerating large-scale language models on distributed system has attracted a lot of attention.
Megatron-LM \cite{shoeybi_megatron-lm_2020} proposes a tensor partitioning strategy for model parallelism that reduces the inter-node communication. 
DeepSpeed \cite{rajbhandari_deepspeed-moe_2022} combines different modes of parallelism to train models with up to a trillion parameters.
\cite{narayanan_efficient_2021} improves pipeline parallelism and combines it with Megatron-LM and achieves high aggregate throughput.
PaLM \cite{chowdhery_palm_2022} is a 540B parameter model trained on 6144 TPU v4 chips using Pathways \cite{barham_pathways_2022}.

\section{Conclusion}
\label{sec:con}

In this work, we propose Chiplet Cloud, a cloud-scale chiplet architecture that optimizes large language model inference.
We discuss the benefits and costs of different mapping strategies.
We propose a design flow that searches and evaluates the design space and outputs the design with the optimal cost, power, or TCO.
With this flow, we designed Chiplet Cloud servers for four language models of different sizes and achieved up to $490 \times$ better performance per TCO versus GPUs.
We believe Chiplet Cloud and all the analysis and discussion in this paper will help the deployment of large language models.

